Continual Learning of Unsupervised Monocular Depth from Videos

Spatial scene understanding, including monocular depth estimation, is an important problem in various applications, such as robotics and autonomous driving. While improvements in unsupervised monocular depth estimation have potentially allowed models to be trained on diverse crowdsourced videos, this remains underexplored as most methods utilize the standard training protocol, wherein the models are trained from scratch on all data after new data is collected. Instead, continual training of models on sequentially collected data would significantly reduce computational and memory costs. Nevertheless, naive continual training leads to catastrophic forgetting, where the model performance deteriorates on older domains as it learns on newer domains, highlighting the trade-off between model stability and plasticity. While several techniques have been proposed to address this issue in image classification, the high-dimensional and spatiotemporally correlated outputs of depth estimation make it a distinct challenge. To the best of our knowledge, no framework or method currently exists focusing on the problem of continual learning in depth estimation. Thus, we introduce a framework that captures the challenges of continual unsupervised depth estimation (CUDE), and define the necessary metrics to evaluate model performance. We propose a rehearsal-based dual-memory method, MonoDepthCL, which utilizes spatiotemporal consistency for continual learning in depth estimation, even when the camera intrinsics are unknown.

==> files/broader_impact.tex <==
\subsubsection*{Broader Impact Statement}
discuss possible repercussions of the work, notably any potential negative impact that a user of this research should be aware of. 
\url{https://jmlr.org/tmlr/ethics.html}

==> files/limitation.tex <==
\section{Limitations}

==> files/todo.tex <==
Add framework to method **
Rewrite background part in method **
Motivation of our method, expand **
Write stc into our cl method part after changing eqn **
Confirm consistency with diagram **

Fix intro **
Fix intro diagram **

Framework diagram ** 
Energy calculation **

stable and plastic are the models and depth and ego-motion are the networks. **

Replace all self-supervised with unsupervised throughout ** 
Ego-motion, not pose. Replace wherever wrong.

use mathcal for stable and plastic model symbols **
resize equations **
stable and plastic are now context and working models **
Add table complete with all stats and buffer sizes **
Finalize related works and Mention ER in related work and/or method. REMOVE SOME OF OUR CITATIONS - REMOVE G2S, TARC, SYNERGY. ADD DUALPROMPT. **
check if we need to cite someone for fwt/bwt/spto. 

Captions - ??
RESULTS - ??


%APPENDIX



-----------------------
change the framework task headings shape and remove arrow of tasks

commas and full stops in eqns

remove the khan paper citation - this is in related works

Change to naive continual training and change MOnodepthCL to Continual Training protocol in Fig 1 **

Change to Working Model and Context Model **

algorithm comments should come after the math/method/step ** 

%CORL

pass through grammarly premium

State what's in appendix in the main text. 

Replace Appendix with Supplementary Material

-------------------

Potentially move the architecture and hyperparams, framework details to appendix. **
Metric details at bare minimum in the main text with details in appendix.  **
Depth Estimation method can perhaps be moved 90\% to the appendix, with just the summary in the main text. **
settings description complete including warmup **
Ablations of warmup and cropping in appendix **
Hyper-param analysis in appendix ** xx
check s-> t or t-> s **
Mention whether stable or plastic is being used **
Cite SPTO **xx
- switch to american english **
Mention commoda buffer being different in related works **xx
Limitations **
Change text to reflect why classification methods aren't immediately extensible to unsupervised depth **
